Encyclopedic VQA: Visual questions about detailed properties of fine-grained categories

We propose Encyclopedic-VQA, a large scale visual question answering (VQA) dataset featuring visual questions about detailed properties of fine-grained categories and instances. It contains 221k unique question+answer pairs each matched with (up to) 5 images, resulting in a total of 1M VQA samples. Moreover, our dataset comes with a controlled knowledge base derived from Wikipedia, marking the evidence to support each answer. Empirically, we show that our dataset poses a hard challenge for large vision+language models as they perform poorly on our dataset: PaLI [14] is state-of-the-art on OK-VQA [37], yet it only achieves 13.0% accuracy on our dataset. Moreover, we experimentally show that progress on answering our encyclopedic questions can be achieved by augmenting large models with a mechanism that retrieves relevant information from the knowledge base. An oracle experiment with perfect retrieval achieves 87.0% accuracy on the single-hop portion of our dataset, and an automatic retrieval-augmented prototype yields 48.8%. We believe that our dataset enables future research on retrieval-augmented vision+language models. It is available at https://github.com/google-research/google-research/tree/master/encyclopedic_vqa .

==> 05_exp_notes.tex <==

\lluis{Number of WIKI articles with title and images: 1234154.}

\lluis{Number of images in the knowledge base: 3009511.}

\begin{table*}[t]
    \centering
    \begin{tabular}{l|c|c|c|c}
        \toprule
        Model & Backbone & Input & Context & VQA Accuracy \\
        \midrule
        KAT & T5-Large & Text + Context + GPT-3 & Wikidata entity + description & 53.09 \\ 
        REVEAL & T5-Large + ViT-g/14 & Text + Context & Wikidata + WIT + VQAv2 + CC12M &  59.1 \\ 
        \midrule
        FLAN-U-PaLM & PaLM 540B & Text & -          & 17.49 \\ 
        FLAN-U-PaLM & PaLM 540B & Text + Context & Wikidata entity + description & 20.33 \\
        PaLI &  ViT-e + T5-XXL & Image + Text & -          & \textbf{64.50} \\ 
        PaLI &  ViT-e + T5-XXL & Image + Text + Context & Wikidata entity + description & 42.64 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{OK-VQA results:}}
    \label{tab:okvqa_results}
\end{table*}



    









\begin{table}[t]
        \centering
        \begin{tabular}{c|c|c}
            \toprule
             & \textbf{PaLI} & \textbf{Flan-PaLM} \\
            \midrule
            Multi-answer & 0.02 & 0.05 \\ 
            Multi-hop &  6.9 &  9.8 \\ 
            \bottomrule
        \end{tabular}
        \caption{\textbf{State-of-the-art for OK-VQA:} We report the best VQA models for OK-VQA. While knowledge retrieval can improve the results of vision and language models, using large multimodal models trained on large amounts of data beats retrieval-based setups significantly.}
        \label{tab:okvqa_results}
    \end{table}





==> 05_table_ablation.tex <==
\newcommand{\rotatecell}[1]{%
    \rotatebox[origin=c]{90}{%
        \begin{tabular}{@{}c@{}}\textbf{#1}\end{tabular}}
    }

\begin{table}[t]
    \centering
    \vspace{-.0cm}
    \begin{adjustbox}{max width=\columnwidth}
    \begin{tabular}{cl@{}l@{}rrrr}
    \toprule
    \multicolumn{1}{l}{}  &                    &                      & \multicolumn{2}{c}{\textbf{Templated}} & \multicolumn{2}{c}{\textbf{Automatic}}\\
    \cmidrule(lr){4-5}\cmidrule(lr){6-7}
    \multicolumn{1}{l}{}  & \textbf{Retriever} & & \multicolumn{1}{c}{\textbf{iNat21}} & \multicolumn{1}{c}{\textbf{GLDv2}} & \multicolumn{1}{c}{\textbf{iNat21}} & \multicolumn{1}{c}{\textbf{GLDv2}} \\    
    \midrule
    \multirow{3}{*}{\rotatecell{PaLI}} & -   && 5.4 & 3.6 & 18.5 & 13.2 \\
                          & Lens -- KB Article && 8.8 & 21.2 & 26.3 & 20.6 \\
                          & Lens -- KB Section && 10.6 & 22.8 & 35.3 & 28.7 \\ 
                          \midrule
    \multirow{3}{*}{\rotatecell{PaLM}} & -  && 6.8 & 5.8 & 28.1 & 20.2 \\
                          & Lens -- KB Article && 33.6 & 42.6 & 52.1 & 50.9 \\
                          & Lens -- KB Section && 33.2 & 41.6 & 53.5 & 52.4 \\
                          \midrule
    \multirow{3}{*}{\rotatecell{GPT-3}} & -  && 4.8 & 2.0 & 21.5 & 17.8 \\
                          & Lens -- KB Article && 34.0 & 41.2 & 49.3 & 45.5 \\
                          & Lens -- KB Section && 30.8 & 39.6 & 49.3 & 46.5 \\
                          \bottomrule
    \end{tabular}
    \end{adjustbox}
    \vspace{-2mm}
    \caption{\small \textbf{Single-hop accuracy by question type.} We break down the accuracy of large models for single-hop templated and automatically generated questions. \lluis{Table updated. Jasper and I propose to kill this table or move it to appendix.}}
    \label{tab:ablation_single_hop}
    \vspace{-.3cm}
\end{table}













==> 05_table_all_in_one.tex <==
\renewcommand{\rotatecell}[1]{%
    \rotatebox[origin=c]{90}{%
        \begin{tabular}{@{}c@{}}\textbf{#1}\end{tabular}}
    }

\begin{table*}
    \begin{subtable}[t]{.33\textwidth}        
        \centering
        \begin{adjustbox}{max width=.9\columnwidth}
        \begin{tabular}{ccrr}
        \toprule
        \multicolumn{2}{c}{\textbf{Retrieval}}      & \\ 
        Mechanism               & Information & \textbf{PaLI~\cite{chen22arxiv}}   & \textbf{PaLM~\cite{chowdhery22arxiv}} \\\cmidrule(lr){1-4}
        -                       & -           & 7.8\%           & 10.1\%        \\\cmidrule(lr){1-4}
        \multirow{3}{*}{Oracle} & Subject $C$ & 10.1\%          & 19.0\%        \\
                                & KB Article  & 22.5\%          & 52.2\%        \\
                                & KB Section  & 37.5\%          & 79.4\%        \\\cmidrule(lr){1-4}
        \multirow{2}{*}{Lens}   & KB Article  & 15.6\%          & 33.3\%        \\
                                & KB Section  & 22.2\%          & 42.0\%        \\ \bottomrule
        \end{tabular}
        \end{adjustbox}
        \caption{\small \textbf{One-hop Accuracy.} We report model accuracy for one-hop templated and automatically generated questions. While large models struggle with our \kivqa dataset, oracle experiments as well as our proof-of-concept Lens retriever show the promise of augmenting large models with a retrieval mechanism on a knowledge base.
        }
        \label{tab:kivqa_results}
    \end{subtable}    
    \begin{subtable}[t]{.33\textwidth}
        \centering
        \begin{adjustbox}{max width=\columnwidth}
        \begin{tabular}{ccccc}
        \toprule
        & \multicolumn{3}{c}{\textbf{Accuracy}} & \\ \cmidrule(lr){2-4}    
        & & w/ correct & w/ incorrect & \textbf{KB retrieval}\\
        \textbf{Lens Retrieval} & Overall & retrieval & retrieval & \textbf{accuracy} \\ \midrule    
        KB Article & 33.3\%            & 52.8\%            & 14.3\%               & 54.9\%        \\
        KB Section & 42.1\%            & 70.0\%            & 10.7\%               & 52.9\%        \\ \bottomrule
        \end{tabular}
        \end{adjustbox}
        \caption{\small \textbf{Attribution for retrieval-augmented VLMs}. We report model accuracy for PaLM~\cite{chowdhery22arxiv} conditional on retrieval results. Retrieval success rates are similar retrieving articles or sections, but PaLM has better accuracy when augmented with sections.}
        \label{tab:attribution_results}
    \end{subtable}
    ~
    \begin{subtable}[t]{.33\textwidth}
        \centering
        \begin{adjustbox}{max width=\columnwidth}
        \begin{tabular}{cl@{}l@{}rrrr}
        \toprule
        \multicolumn{1}{l}{}  &                    &                      & \multicolumn{2}{c}{\textbf{Templated}} & \multicolumn{2}{c}{\textbf{Automatic}}\\
        \cmidrule(lr){4-5}\cmidrule(lr){6-7}
        \multicolumn{1}{l}{}  & \textbf{Retriever} & & \multicolumn{1}{c}{\textbf{iNat'21}} & \multicolumn{1}{c}{\textbf{GLDv2}} & \multicolumn{1}{c}{\textbf{iNat21}} & \multicolumn{1}{c}{\textbf{GLDv2}} \\    
        \midrule
        \multirow{3}{*}{\rotatecell{PaLI}} & -   && 3.7 & 2.0 & 9.4 & 7.4 \\
                              & Lens -- KB Article && 6.9 & 23.1 & 16.2 & 15.4 \\
                              & Lens -- KB Section && 8.5 & 25.9 & 24.1 & 21.6 \\ 
                              \midrule
        \multirow{3}{*}{\rotatecell{PaLM}} & -  && 5.5 & 3.6 & 13.5 & 8.0 \\
                              & Lens -- KB Article && 14.4 & 38.5 & 32.3 & 36.0 \\
                              & Lens -- KB Section && 19.3 & 36.1 & 46.7 & 41.0 \\
                              \bottomrule
        \end{tabular}
        \end{adjustbox}
        \caption{\small \textbf{Single-hop accuracy by question type.} We break down the accuracy of large models for single-hop templated and automatically generated questions.} \label{tab:ablation_single_hop}
    \end{subtable}    
\end{table*}

==> A0_abstract.tex <==
\begin{abstract}
In this supplementary material, we provide additional details to our submission.
We present the specific prompts that were used for large language (PaLM) and vision+language (PaLI) models.
Additionally, we present qualitative results for the different techniques that were evaluated on our questions.

\end{abstract}

==> rw_notes_not_part_of_paper.tex <==

\section{Related work notes on datasets - Not part of actual paper.}
\label{sec:related_work_notes}

\para{OK-VQA.} Dataset collection: (1) Ask annotators to write a question given an image. (2) Manually (!) filter the 86700 questions to require outside knowledge. (3) Remove biased questions (e.g. all answered 'yes' or 'winter').

\para{A-OKVQA.} Dataset collection: The A-OKVQA dataset is meant to require more common-sense knowledge than the OK-VQA dataset (e.g. beyond simple lookup questoins) and requires more complex reasoning. In particular, they require visual knowledge (44\% of the questions), common-sense knowledge (36\%), knowledge base (18\%), and physical knowledge (3\%). In addition, they also provide rationales. Finally, they have a multiple-choice mode in addition to the open question mode. The process of collecting questions is: (1) Ask annotators to write questions given an image. They have a training and selection procedure in place in order to get questions which (a) require looking at the image, (b) require common-sense knowledge or specialized knowledge, (c) requires thinking beyond recognizing the object, and (d) not be too similar to previous questions (which is done by showing the rater related questions for similar images using CLIP).
Next, (2) All questions were screened by three workers and only were included if the majority decided it was a good question (eliminating 60\% of the questions). (3) nine additional free-form answers were given by a different pool of workers. (4) for each question three rationales were collected.

\para{VQAv1} data collection: (1) Human annotators were asked to create questions given an image, where a smart prompt was used to prevent annotators asking trivial questions (i.e. (paraphrased) ask a question which a human can easily answer but a robot who can recognize all objects in the image cannot easily answer). (2) 10 open-ended answers were collected for each question. \jasper{@Thomas: Before comparison, all responses are made lowercase, numbers converted to digits, and punctuation \& articles removed.}
\jasper{@Lluis: The VQAv1 metric where they report accuracies averaged over $10 \choose 9$ sets was done to be able to compare to human accuracies.}

\para{VQAv2} data collection: They authors want to reduce language bias in V1 by having questions whose answer changes based on the image. To do so, they take existing Q/A/I triplets from VQAv1, take the 24 nearest neighbour images, and ask annotators to select an image for which Q makes sense but for which A is not the correct answer. These new Q+I pairs are then send to annotators to obtain 10 answers for each pair.
\jasper{Another possibility would have been to exclude questions which can be based on the question alone given an LLM. Note that this is one of our design principles and established by the templated questions. We can do a rough analysis for automatically generated questions by looking at the question groupings which I made for the comparative questions.}

\para{FM-IQA~\cite{gao15neurips}.} They start with 158k COCO images. Annotators are asked to ask any type of questions related to the content of images. Questions should be answerable using visual content and common sense knowledge. Quality 'curated' by selecting annotators who ask interesting questions as judged by the authors. Fig 3. shows mostly trivial VQA examples:
\vitto{well, rather than 'trivial', I'd say these examples need only the image and commonsense knowledge, as opposed to requiring a KB / encyclopedic / fine-grained knowledge.}
what is the boy in green doing? Is there a person in the image? is the computer on the left hand side or right hand side of the gentleman? Why does the bus park here? Is the man trying to buy vegetables? How many layers are there fore the case? What is the color of the bus? What is on the grass besides a person?

\para{VCR~\cite{zellers19cvpr}}. QA pairs on asking questions for commonsense visual reasoning about the visual world. Created on top of images from movies. Dataset includes rationales. A lot of this dataset is about understanding of social situations. Dataset is multiple-choice where the non-correct options are created adversarially.

\para{S3VQA~\cite{jain21sigir}}.
\vitto{the opening para of this paper has a greatly phrased attack to OK-VQA. We should reuse some of that attack ourselves.}
One part is based on OKVQA. More interesting is the S3VQA dataset itself. They use OpenImages. For each object they identify a parent category (e.g. peacock maps to bird). They semi-automatically find the appropriate wikipedia page for peacock. Then they automatically generate a QA pair from the wikipedia page using a model based on T5 model (they cite T5~\cite{raffel21jmlr}, not a specific QA generation sytem). They only retain the QA pairs for which Q explicitly mentions the object of interest (i.e. peacock in the example). They claim that by design, and unlike OK-VQA, a question only has one unique correct answer.
\vitto{they also claim that 'every question is guaranteed to require integration of the knowledge-base.' If true, this is a distinguishing feature over OK-VQA, and makes it nearer to our dataset. We should pick up on that. The idea of having a super-class named in the question, rather than the exact class in the image, is core in our dataset as well.}
Afterwards, they generalize the question by replacing the entity with its supercategory (e.g. peacock becomes bird). Then the authors manually filtered questions for which only the image was needed and manually improved grammar for questions where necessary. Finally, they generated paraphrases versions of these questions with T5 and pegasus~\cite{zhang20icml} which were selected by human annotators as alternatives.
\vitto{overall, from my checking of the paper, this is perhaps the most related dataset. We should dedicate a bit more space to it in our rel work section than to other datasets. We still have at least two major advantages: (1) our dataset is much bigger; (2) we have multi-hop, instead of just single-hop.}

\para{DAQUAR~\cite{malinowski14neurips}}. They collect QA pairs on the NYU dataset. They have 'synthetic questions' which are templated questions which are about counting, colors, room type, comparisons (which is the largest X in the image). They have also human-collected QA pairs where they restrict the answer to be colours, numbers, or object categories, or any combinations of those. Basically, all information is truly in the image itself. DAQUAR is probably one of the first VQA datasets.

\para{KB-VQA~\cite{wang17ijcai}}. The authors define templates. They choose 700 images from COCO val. Then they ask experts to generate 3-5 QA pairs for each of the 700 images based on the predefined templates (e.g. IsThereAny, IsImgRelate, WhatIs, ImgScene, ColorOf, etc.) They divide the templates into three types of questions: visual, common-sense, or KB-knowledge. They get 1256, 883, and 263 questions for these types respectively. In contrast, they claim that for the VQAv1 dataset only 5.5\% of the questions require common-sense while none require KB-knowledge. \vitto{hum, a bit unclear: so 263 questions require a KB (and hence are related to our work). But then you say none. I guess these two statements refer to two different datasets, but which ones?}\jasper{Fixed. The 263 is about KB-VQA, the other statement is about VQAv1. Note that I removed this dataset from the related work completely since FVQA is mostly from the same authors and seems an improvement.}

\para{FVQA~\cite{wang18pami}}. Same authors as KB-VQA. Again the claim about VQAv1: 5.5\% of the VQA dataset requires adult-level knowledge, 11.2\% requires teenager-level knowledge, and 28.4\% requires older-child knowledge (9-12). In this paper they double down on the requirement for a knowledge base. However, they call the type of knowledge 'common-sense' knowledge since the facts are from DBpedia, ConceptNet, and WebChild; the type of relationships are category, relatedTo, capableOf, UsedFor (lighthouse is used for SignalingDanger), HasProperty (wedding HasProperty romantic), createdBy (bread CreatedBy Flour), Smaller, Better (Apple Better VitaminPill), Taller. Furthermore, answers are required to be in the knowledge base. The database is provided with the dataset in the form of triplets.

\para{KVQA~\cite{shah19aaai}}. They harvest persons+images from wikipedia. They only keep images with humans there. They have raters ask a list of templated questions. From these they wrote SPARQL queries to obtain the answers. Finally, they have an online tool to paraphrase the questions (but they provide both the original and paraphrased questions). They provide the wikimedia triplets which are used to extract the knowledge. 
\vitto{overall it seems like the rel work srtructure you have now will work: first a para on VQA datasets that really only require looking at the image and maybe some common sense reasoning. Then a longer para those that (claim to) require some form of external knowledge, to various degrees. Perhaps ordered by how much we believe they really need an actual KB. }

\para{HotpotQA~\cite{yang18emnlp}}. They create a QA dataset from wikipedia. They look at the first paragraph and find all hyperlinks. They create a graph using these hyperlinks. They manually define a set of bridge entities (591 categories from the list of popular pages by WikiProject). For every edge (a, b) where $b$ is a bridge entity they show the two top-paragraphs of wikipedia and ask annotators to create a question which requires information from both paragraphs. They also ask comparative questions as follows: they first look at the 'list of lists of lists' page of wikipedia, from which they manually identify 42 lists of similar entities. Then they take two entities within a list and ask annotators for a comparative question (e.g. are Iron Maiden and AC/DC from the same country?). They also annotate supporting evidence, which are single sentences within a wikipedia section.
In the end, they identify different required reasoning types: (Comparison) comparing two entities (20\%). (Type-I) Chaining bridge entities (38\%) (which is what we do). (Type-II) Locating the answer by checking multiple properties (29\%) (e.g. combining a list with a property; translated in the context of our paper an example would be 'which of these animals hunts deer?'. (Type-III) Inferring a property of an entity through a bridge entity (2\%). E.g. translated to our domain: 'on which continent does this animal live?' where 'Italy' is a bridge entity. (Single-hop) - 2\%. (Unanswerable) - 2\%.

Note: They have an interesting plot with answer-types: Fig. 2: \url{https://aclanthology.org/D18-1259.pdf}.
They differentiate themselves from QAngaroo and ComplexWebQuestions sincs these two works create multi-hop questions from DB triplets rather than free-form text.

\subsection{Reasoning for open-world answers choice in Tab. \ref{tab:my_label}}

\paragraph{OK-VQA}. The methods used in the paper classify answers into 2000 possible classes. They report that 88.5\% of questions in the test set are covered by the top 2000 answers.

\paragraph{A-OKVQA}. They experiment with generative models to produce answers, such as GPT-3 and ClipClap. 
For models with classification prediction, they use the top 10,424 answers from the training set as vocabulary.
Most training answers appear in the train/val/test splits, from their paper: 

``We find that in the val set, the ground-truth answer for 87.6\% of questions appears in the train set while in the test set 82.7\% do. This shows that there is indeed some reasonable similarity between the sets, but also that a significant portion of the held out sets require an answer that the model will not have seen during training, requiring the model to be able to generate out-of-distribution answers or generate answers based on some knowledge outside of the dataset.''

So, taking the top answers in the training set could work reasonably well in A-OKVQA. Or, even just using a 25k-sized vocabulary would be enough, since there are fewer answers than this. In theory, if the model is well-learned, then the model could get 82.7\% accuracy.

BTW, S3VQA does a frontal atack on OKVQA due to this: 

[on OKVQA] ``frequency-based guessing is very effective because of (unintended) widespread answer overlaps between train and test folds.''

\paragraph{S3VQA}.
It's likely that this dataset really has open-world answers, since questions are generated from Wikipedia using T5, similar to our data collection process.
Even though the visual data is high-level (coming from OpenImages), the specificity of the answers is likely high.
However, they don't seem to have statistics on this.

\paragraph{FVQA}
Vocabulary seems limited to concepts in the query images and in the knowledge triplets. But hard to tell exactly, since they don't present statistics of answer overlap between train and test splits.

`` the answer to a visual question in our collected dataset can be either the visual concept in the supporting-fact (i.e., ?X), or the other concept on the KB side (i.e., ?Y).''


\paragraph{KVQA}. They report the following:

``Number of QA pairs 183,007''

``Number of unique answers 19,571''

So there's on average one answer for every 9.3 questions. So it seems like there is likely a lot of overlap. They show a word cloud in fig 4 as well. Their experiments are with a classifier to predict the answers, but they don't seem to say how many classes are there. InFactuality also uses a classification head and achieves high performance.



